The Blending Ratio Is Not Where the Performance Is: Diagnosing Prototype Blending for Few-Shot Adaptation of Vision-Language Models

Many few-shot adaptation methods for vision-language models classify with a convex combination of the zero-shot text prototype and the mean of the K labelled image features, with a single blending ratio routinely tuned on held-out labels, often on the test set itself. We ask what the family's own bias-variance justification invites: what is the right ratio, can it be estimated without validation data, and is finding it where the performance is? First, the ratio minimising prototype mean-squared error has a closed form whose support-set plug-in is exactly a positive-part James-Stein coefficient shrinking towards the text prototype. Across 4,800 cells (ten datasets, five backbones including SigLIP, five shot counts, five seeds, four prompt tiers) this theoretically optimal ratio is a reliable estimate of the wrong quantity: on the 950 primary-tier cells where it is defined it trails a test-set-oracle ratio by 8.5 points. It saturates near 1, discarding the text prior for a nearest-class-mean classifier, because 78% of the text-image prototype distance it treats as bias is a class-independent offset that the arg max largely cancels. We prove the mechanism and bound its share of the damage at 26% by a counterfactual. Second, leave-one-out on the support set alone sets a ratio landing within 0.9 points of the oracle blend, so it is estimable without validation data. Third, validation-free linear probes beat even the oracle-tuned blend: CLAP by +1.9 points and LP++ by +1.5 on average, and at K >= 4 all four validation-free baselines sit above the oracle, the linear probes by margins excluding zero. These results locate the ceiling in the model class, not the hyperparameter: the ratio can be set near-optimally for free, and it is still not where the performance is. Code, cached features, per-cell records: https://huggingface.co/datasets/Liangzhi-Li/clipbench-blending

==> tables/aug.tex <==
\begin{table}[t]
\caption{Effect of restoring the official image-augmentation pipelines
(20-view random-resized-crop + flip caches; Sec.~\ref{sec:protocol}), as the
paired per-cell accuracy difference \emph{augmented $-$ cached-only} (pp,
cluster-bootstrap 95\% CI). Cells, support draws, and test sets are identical
to the main matrix. Bold: CI excludes zero. Coverage: 39 of the 50 (dataset, backbone) pairs of the full grid, with RN50, ViT-B/16 on every dataset; the paired contrasts are unaffected, the intervals wider than a complete grid's.}
\label{tab:aug}
\centering\scriptsize
\setlength{\tabcolsep}{2.2pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l cccc}
\toprule
Method & all $K$ & $K{=}1$ & $K{=}2$ & $K\ge4$\\
\midrule
CLAP & -0.08 [-0.52, +0.36] & \textbf{+0.27 [+0.00, +0.55]} & -0.04 [-0.64, +0.55] & -0.26 [-0.74, +0.23] \\
LP++ & -0.98 [-2.13, +0.18] & -0.82 [-1.82, +0.18] & -1.04 [-2.45, +0.36] & -1.02 [-2.20, +0.16] \\
HOSO & \textbf{+0.28 [+0.04, +0.52]} & -- & +0.23 [-0.16, +0.62] & \textbf{+0.30 [+0.07, +0.53]} \\
GDA ($\alpha{=}1$) & \textbf{-3.00 [-5.68, -0.32]} & \textbf{-18.83 [-30.66, -6.99]} & \textbf{+4.27 [+1.18, +7.36]} & +0.93 [-0.40, +2.26] \\
GDA ($\alpha$-LOO) & \textbf{-3.60 [-6.52, -0.68]} & \textbf{-18.83 [-30.66, -6.99]} & \textbf{+3.17 [+0.97, +5.36]} & +0.28 [-1.03, +1.60] \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/coop.tex <==
\begin{table}[t]
\caption{The three findings replicated on the CoOp \texttt{split\_zhou}
protocol (nine shared datasets plus UCF101; ImageNet excluded as its CoOp
variant requires the full training set). Paired within-cell differences,
cluster-bootstrap 95\% CIs, dataset-specific prompt. Coverage: 23 of the 50 (dataset, backbone) pairs of the full grid, with ViT-B/16 on every dataset; the paired contrasts are unaffected, the intervals wider than a complete grid's.}
\label{tab:coop}
\centering\scriptsize
\setlength{\tabcolsep}{2.2pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l cc cc}
\toprule
 & \multicolumn{2}{c}{All $K$} & \multicolumn{2}{c}{$K\ge4$}\\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
Contrast & $\Delta$ [95\% CI] & $n$ & $\Delta$ [95\% CI] & $n$\\
\midrule
JS blend $-$ oracle ratio & -7.68 [-13.70, -1.67] & 268 & -5.84 [-11.17, -0.51] & 187 \\
LOO blend $-$ oracle ratio & -1.64 [-2.93, -0.35] & 268 & -1.04 [-1.75, -0.34] & 187 \\
CLAP $-$ oracle ratio & +2.26 [+1.04, +3.49] & 349 & +3.08 [+1.30, +4.87] & 187 \\
LP++ $-$ oracle ratio & +1.92 [+0.21, +3.62] & 349 & +3.67 [+0.91, +6.43] & 187 \\
JS blend $-$ zero-shot & +5.86 [-8.00, +19.72] & 268 & +8.94 [-4.75, +22.62] & 187 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/gapshare.tex <==
\begin{table}[t]
\caption{Share of the squared text--image prototype distance $\smash{\|\boldsymbol{\mu}_t-\boldsymbol{\mu}^*\|^2}$ that is \emph{class-independent} (\%, cluster-bootstrap 95\% CI over the ten datasets; $n{=}4{,}800$ cells). This component is constant across classes and cancels in the arg\,max, yet the MSE objective of Eq.~\eqref{eq:mse} charges it to the text prototype as ``bias''.}
\label{tab:gapshare}
\centering\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l cc}
\toprule
Backbone & Class-indep.\ share (\%) & 95\% CI\\
\midrule
RN50 & 73.9 & [68.3, 79.4] \\
ViT-B-32 & 77.6 & [73.2, 82.0] \\
ViT-B-16 & 78.0 & [73.8, 82.2] \\
ViT-L-14 & 75.7 & [72.0, 79.3] \\
SigLIP-B-16 & 86.6 & [84.6, 88.6] \\
\midrule
All backbones & 78.3 & [74.6, 82.1] \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/perclass.tex <==
\begin{table}[t]
\caption{Is the ceiling an artefact of allowing only \emph{one} blending ratio?
Paired differences (pp, cluster-bootstrap 95\% CI over datasets) on ViT-B/16,
ten datasets $\times$ five shot counts $\times$ three seeds. A per-class oracle
fits $C$ ratios to the labels it is scored on, so its in-sample gain mixes
capacity with memorisation; the split-half row separates them. Even the honest
per-class oracle is beaten by a validation-free linear probe.}
\label{tab:perclass}
\centering\scriptsize
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l cc}
\toprule
Contrast & $\Delta$ [95\% CI] & $n$\\
\midrule
Per-class oracle $-$ global oracle (fitted \emph{and} scored on test) & +1.52 [+0.36, +2.68] & 144 \\
Per-class oracle $-$ global oracle (fit on half the test set, scored on the other) & -0.52 [-2.24, +1.20] & 144 \\
CLAP $-$ per-class oracle (held-out) & +2.18 [+0.17, +4.20] & 144 \\
LP++ $-$ per-class oracle (held-out) & +2.16 [+0.23, +4.09] & 144 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/precision.tex <==
\begin{table}[t]
\caption{float64 vs.\ float32 solver precision: absolute accuracy difference (pp) on identical support sets, over the eight dataset$\times$backbone shards computed in both precisions. Only HOSO is materially precision-sensitive; its results should be read with a ${\sim}0.5$\,pp band.}
\label{tab:precision}
\centering\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l ccc}
\toprule
Method & $n$ cells & mean $|\Delta|$ & max $|\Delta|$\\
\midrule
hoso & 160 & 0.439 & 3.093 \\
lp++ & 200 & 0.006 & 0.106 \\
zeroshot & 800 & 0.000 & 0.000 \\
ncm & 800 & 0.000 & 0.000 \\
all 11 remaining methods & 5160 & 0.000 & 0.000 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/robust.tex <==
\begin{table}[t]
\caption{Two protocol objections, measured. \emph{(a)} paired accuracy change from restoring each
method's official image-augmentation recipe on a seeded 20-view support cache, against the
cached-only main matrix, on identical cells. \emph{(b)} the headline contrasts recomputed after
re-extracting every feature on the CoOp \texttt{split\_zhou} splits (UCF101 included, ImageNet
excluded). All entries are pp with cluster-bootstrap 95\% CIs over datasets; bold excludes zero.}
\label{tab:robust}
\centering\scriptsize
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l cc}
\toprule
 & all $K$ & $K{=}1$ \slash $K{\ge}4$\\
\midrule
\multicolumn{3}{l}{\itshape (a) restoring each official augmentation recipe ($n{=}817$ paired cells)}\\
\quad CLAP & -0.08 [-0.52, +0.36] & \textbf{+0.28 [+0.00, +0.55]} \\
\quad LP++ & -0.98 [-2.13, +0.18] & -0.82 [-1.82, +0.18] \\
\quad HOSO & \textbf{+0.28 [+0.04, +0.52]} & -- \\
\quad GDA ($\alpha{=}1$) & \textbf{-3.00 [-5.68, -0.32]} & \textbf{-18.83 [-30.66, -6.99]} \\
\midrule
\multicolumn{3}{l}{\itshape (b) re-extracting on the CoOp \texttt{split\_zhou} protocol ($n{=}349$ cells)}\\
\quad CLAP $-$ oracle $\lambda$ & \textbf{+2.26 [+1.04, +3.49]} & \textbf{+3.08 [+1.30, +4.87]} \\
\quad LP++ $-$ oracle $\lambda$ & \textbf{+1.92 [+0.21, +3.62]} & \textbf{+3.67 [+0.91, +6.43]} \\
\quad LOO blend $-$ oracle $\lambda$ & \textbf{-1.64 [-2.93, -0.35]} & \textbf{-1.04 [-1.75, -0.34]} \\
\quad JS blend $-$ oracle $\lambda$ & \textbf{-7.68 [-13.70, -1.67]} & \textbf{-5.84 [-11.17, -0.51]} \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/taxonomy.tex <==
\begin{table}[t]
\caption{Method taxonomy. ``VF'' = validation-free as run here: fits using only the $K$ support shots and the class names. ``Selected quantity'' names the trust hyperparameter each method must set and how it is set in our protocol. Daggered rows are reference bounds, not methods.}
\label{tab:taxonomy}
\centering\scriptsize
\setlength{\tabcolsep}{2.6pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l l l c}
\toprule
Method & Model class & Selected quantity & VF\\
\midrule
Zero-shot & text prototypes & --- & \checkmark\\
NCM & image prototypes & --- & \checkmark\\
JS blend, Eq.~\eqref{eq:jshat} & blended prototypes & $\lambda_c$ closed form & \checkmark\\
Centred JS & blended prototypes & $\lambda_c$ closed form & \checkmark\\
LOO blend (Sec.~\ref{sec:estimation}) & blended prototypes & global $\lambda$ by LOO & \checkmark\\
GDA ($\alpha{=}1$)~\cite{wang2024gda} & GDA + ZS logits & $\alpha$ fixed & \checkmark\\
GDA ($\alpha$ by LOO) & GDA + ZS logits & $\alpha$ by LOO & \checkmark\\
HOSO~\cite{vorster2026hoso} & adapter + blend & ratio on 1 held shot & \checkmark\\
CLAP~\cite{silva2024closer} & linear probe & multipliers by ALM & \checkmark\\
LP++~\cite{huang2024lppp} & linear probe + text & step sizes analytic & \checkmark\\
\midrule
GDA (official)$^\dagger$~\cite{wang2024gda} & GDA + ZS logits & $\alpha$ on val.\ labels & --\\
Oracle $\lambda$$^\dagger$ & blended prototypes & global $\lambda$ on test & --\\
Tip-Adapter$^\dagger$~\cite{zhang2022tip} & cache + ZS logits & $\alpha,\beta$ on test & --\\
MSE-oracle$^\dagger$, Eq.~\eqref{eq:lamstar} & blended prototypes & $\lambda_c^*$ from pool & --\\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/vs_loo.tex <==
\begin{table}[t]
\caption{Paired accuracy difference (pp, 95\% CI) of each method relative to the LOO blend. Positive = better than the LOO blend.}
\label{tab:vsloo}
\centering\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l c c}
\toprule
Method vs.\ LOO blend & $\Delta$ [95\% CI] & $n$\\
\midrule
CLAP & +3.05 [+1.51, +4.59] & 950 \\
LP++ & +3.03 [+1.29, +4.77] & 950 \\
HOSO & +1.18 [-0.03, +2.39] & 950 \\
GDA ($\alpha$ by LOO) & +0.63 [-2.16, +3.41] & 950 \\
GDA ($\alpha{=}1$) & -1.42 [-5.03, +2.19] & 950 \\
James--Stein blend & -7.70 [-12.51, -2.88] & 950 \\
Zero-shot & -7.58 [-12.43, -2.73] & 950 \\
\bottomrule
\end{tabular}
}
\end{table}

